NP-Logic Systems and Model-Equivalence Reductions

In this paper we investigate the existence of model-equivalence reduction between NP-logic systems which are logic systems with model existence problem in NP. It is shown that among all NP-systems with model checking problem in NP, the existentially quantified propositional logic (\exists PF) is maximal with respect to poly-time model-equivalent reduction. However, \exists PF seems not a maximal NP-system in general because there exits a NP-system with model checking problem D^P-complete.

==> eptcsdata.tex <==
\providecommand{\event}{X. Zheng and N. Zhong (Eds.)\\
Computability and Complexity in Analysis (CCA 2010)}
\providecommand{\volume}{24}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{130}
\providecommand{\eid}{17}

